Graph Neural Networks for Decentralized Multi-Robot Path Planning

Effective communication is key to successful, decentralized, multi-robot path planning. Yet, it is far from obvious what information is crucial to the task at hand, and how and when it must be shared among robots. To side-step these issues and move beyond hand-crafted heuristics, we propose a combined model that automatically synthesizes local communication and decision-making policies for robots navigating in constrained workspaces. Our architecture is composed of a convolutional neural network (CNN) that extracts adequate features from local observations, and a graph neural network (GNN) that communicates these features among robots. We train the model to imitate an expert algorithm, and use the resulting model online in decentralized planning involving only local communication and local observations. We evaluate our method in simulations {by navigating teams of robots to their destinations in 2D} cluttered workspaces. We measure the success rates and sum of costs over the planned paths. The results show a performance close to that of our expert algorithm, demonstrating the validity of our approach. In particular, we show our model's capability to generalize to previously unseen cases (involving larger environments and larger robot teams).

==> graphConvolution.tex <==
% !TEX root = ../includes.tex

\def \thisplotscale {1.8}
\def \unit {\thisplotscale cm}

\tikzstyle {Phi} = [rectangle, 
                    thin,
                    minimum width = 0.5*\unit, 
                    minimum height = \sumshift*\unit, 
                    anchor = west,
                    draw,
                    fill = pennblue!20]

\tikzstyle {sum} = [circle, 
                    thin,
                    minimum width  = 0.3*\unit, 
                    minimum height = 0.3*\unit, 
                    anchor = center,
                    draw,
                    fill = pennblue!20]


\def \deltax {1.3}
\def \deltay {0.8}
\def \sumshift {0.4}

\begin{tikzpicture}[x = 1*\unit, y = 1*\unit] \footnotesize
    
% Begin by drawing an empty node for initializing the chain
\node (origin) [] {};
\path (origin) ++ (0.2*\deltax, 0) node (first) [] {};
    
% Draw the chain of graph shifts
\path (first) ++ (1.35*\deltax, 0) node (0) [Phi] {$\bbS$};
\path (0)     ++ (1.35*\deltax, 0) node (1) [Phi] {$\bbS$};
\path (1)     ++ (1.35*\deltax, 0) node (2) [Phi] {$\bbS$};

% End by drawing an empty node for finalizing the chain
\path (2.east) ++ (1.0*\sumshift*\deltax, 0) node [anchor=west] (last) [] {};

% Draw the chain of additions
\path (first.east) ++ (1.5*\sumshift*\deltax, -\deltay) node (sum0) [sum] {$+$};
\path (0.east) ++ (\sumshift*\deltax, -\deltay) node (sum1) [sum] {$+$};
\path (1.east) ++ (\sumshift*\deltax, -\deltay) node (sum2) [sum] {$+$};
\path (2.east) ++ (\sumshift*\deltax, -\deltay) node (sum3) [sum] {$+$};

% Draw the arrows connecting the shift blocks
\path[-stealth] (first) edge [very near start, above] node {$\bbx$}               (0);	
\path[-stealth] (0)     edge [above] node {$\ \bbS\bbx$}     (1);	
\path[-stealth] (1)     edge [above] node {$\ \bbS^{2}\bbx$} (2);	
\path[-]        (2)     edge [above, near end] node {$\ \bbS^{3}\bbx$} (sum3 |- last);

% Draw the arrows connecting to the sum blocks
\path[-stealth, draw] (sum0 |- first) -- (sum0) node [midway, right] {$a_{0}$};	
\path[-stealth, draw] (sum1 |- 0)     -- (sum1) node [midway, right] {$a_{1}$};	
\path[-stealth, draw] (sum2 |- 1)     -- (sum2) node [midway, right] {$a_{2}$};	
\path[-stealth, draw] (sum3 |- 2)     -- (sum3) node [midway, right] {$a_{3}$};

% Draw the arrows connecting the sum blocks
\path[-stealth, draw] (sum0) -- (sum1);	
\path[-stealth, draw] (sum1) -- (sum2);	
\path[-stealth, draw] (sum2) -- (sum3);	
                
% % Draw the addition of graph filters
% \path (sum3.east) ++ (1.0*\deltax, 0) node (sumFeatures) [sum, fill=pennred!20] {$+$};
% \path[-stealth,draw] (sum3) -- (sumFeatures) node [midway, above] {$\bbh_{\ell}^{fg} \ast_{\bbS} \bbx_{\ell-1}^{g}$};

% % Draw nonlinearity
% \path (sumFeatures.east) ++ (1.0 * \deltax, 0) node (nonlinearity) [sum, fill=penngreen!20] {$\sigma_{\ell}$};
% \path[-stealth, draw] (sumFeatures) -- (nonlinearity) node [midway, above] {$\displaystyle \sum_{g=1}^{F_{\ell-1}} h_{\ell}^{fg} \ast \bbx_{\ell-1}^{g}$};

% draw output
\path[-stealth] (sum3.east) edge [midway, above] node {$\displaystyle \sum_{k=0}^{K-1} a_{k}\bbS^{k} \bbx$} ++ (\deltax, 0);


\end{tikzpicture}
